Sparsh: Self-supervised touch representations for vision-based tactile sensing

In this work, we introduce general purpose touch representations for the increasingly accessible class of vision-based tactile sensors. Such sensors have led to many recent advances in robot manipulation as they markedly complement vision, yet solutions today often rely on task and sensor specific handcrafted perception models. Collecting real data at scale with task centric ground truth labels, like contact forces and slip, is a challenge further compounded by sensors of various form factor differing in aspects like lighting and gel markings. To tackle this we turn to self-supervised learning (SSL) that has demonstrated remarkable performance in computer vision. We present Sparsh, a family of SSL models that can support various vision-based tactile sensors, alleviating the need for custom labels through pre-training on 460k+ tactile images with masking and self-distillation in pixel and latent spaces. We also build TacBench, to facilitate standardized benchmarking across sensors and models, comprising of six tasks ranging from comprehending tactile properties to enabling physical perception and manipulation planning. In evaluations, we find that SSL pre-training for touch representation outperforms task and sensor-specific end-to-end training by 95.1% on average over TacBench, and Sparsh (DINO) and Sparsh (IJEPA) are the most competitive, indicating the merits of learning in latent space for tactile images. Project page: https://sparsh-ssl.github.io/

==> figures/force_estimation.tex <==
%\begin{wrapfigure}{R}{0.5\textwidth}
%    \includegraphics[width=\linewidth]{figures/force/digit/force_estimation_rmse.png}
%    \caption{\textbf{Force Estimation DIGIT}\todo{caption}}
%    \label{fig:force_performance_digit}
%\end{wrapfigure}
%\begin{wrapfigure}{R}{0.5\textwidth}
%     \includegraphics[width=\linewidth]{figures/force/gelsight/force_estimation_rmse.png}
%    \caption{\textbf{Force Estimation GelSight}\todo{caption}}
%    \label{fig:force_performance_gs}
%\end{wrapfigure}
\GobbleSmall
\begin{wrapfigure}{R}{0.5\textwidth}
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/force/digit/force_estimation_rmse.png}
        %\subcaption{DIGIT}%\todo{caption}}
        \label{fig:force_performance_digit}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/force/gelsight/force_estimation_rmse.png}        %\subcaption{GelSight}%\todo{caption}}
        \label{fig:force_performance_gs}
    \end{subfigure}
    \GobbleSmall
    \vspace{-3mm}
    \caption{RMSE force estimation error vs training data budget for \textbf{[left]} DIGIT and \textbf{[right]} GelSight}
    \label{fig:force_performance}
    \GobbleMedium
    \vspace{-2mm}
\end{wrapfigure}

==> figures/force_field_vis.tex <==
%\GobbleSmall
\begin{wrapfigure}{R}{0.5\textwidth}
    \vspace{-3mm}
    \centering
    \includegraphics[width=\linewidth]{figures/force/fig_force_field_small.pdf}
    \caption{Normalized tactile flow (unitless) visualizations using \dino for key-frames from a representative YCB-Slide (top) and spherical probe (bottom) trajectories. Arrows represent tangential forces, while the colors represent normal forces. 
    }
    \label{fig:force_field_results_dino}
    \GobbleMedium
    \vspace{-3mm}
\end{wrapfigure} 

==> figures/policy_sequence.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{figures/policy/fig_policy.pdf}
    \caption{Keyframes bead maze policy}
    \label{fig:policy-bead-maze}
\end{figure}

==> figures/pose_estimation.tex <==
% \begin{wrapfigure}{r}{0.5\textwidth}
%     \GobbleMedium
%     \includegraphics[width=\linewidth]{figures/pose/relative_pose_estimation2.png}
%     \vspace{-5mm}
%     \caption{Data collection procedure for Pose estimation. We make sure that the allegro lies parallel to the table, facing downward. Sensor observations are obtained from all three primary allegro fingertips, and object poses are obtained by tracking ArUco markers}
%     \label{fig:pose-estimation-benchmark}
%     \GobbleLarge
% \end{wrapfigure}

\begin{wrapfigure}{L}{0.3\textwidth}
    \GobbleLarge
    \centering
    \includegraphics[width=0.8\linewidth]{figures/pose/relative_pose_estimation3.png}
    \vspace{-2mm}
    \caption{Data collection for pose estimation. Sensor observations are obtained from all three primary DIGIT sensors. Object poses are obtained by tracking ArUco markers.}
    \label{fig:pose-estimation-benchmark}
    % \vspace{-10mm}

    \includegraphics[width=\linewidth]{figures/pose/pose_estimation_avg_accuracy.png}
    \caption{Relative pose estimation accuracy vs training budgets.}
    \label{fig:pose_performance_allmodels}
    %\GobbleGiant
    \vspace{-2\baselineskip}
\end{wrapfigure}


==> tables/datasets_ssl.tex <==
% DATASETS FOR SSL 

\begin{table}[h]
\GobbleMedium
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
Dataset          & Sensor             & Size     & Collector \\ \midrule
YCB-Slide~\cite{suresh2022midastouch}        & DIGIT              & 180k     & Human     \\
Touch-Slide      & DIGIT              & 180k     & Human     \\
Touch and Go~\cite{yang2022touch}     & GelSight (markers) & $>13.9$k & Human     \\
ObjectFolder 2.0~\cite{gao2022objectfolder} & GelSight           & $>66$k   & Robot     \\ \bottomrule
\end{tabular}
\caption{\textbf{Tactile Datasets} used for learning tactile representations a. *For all datasets, we incorporate images corresponding to transitions from non-contact to contact.}
\label{tab:datasets_ssl}
\GobbleMedium
\end{table}

% \begin{table}[!t]
% \centering
% \begin{tabular}{@{}cllcll@{}}
% \toprule
% Source &
%   \multicolumn{1}{c}{Dataset} &
%   \multicolumn{1}{c}{Sensor} &
%   Size &
%   \multicolumn{1}{c}{Source} &
%   \multicolumn{1}{c}{Task} \\ \midrule
% \multirow{4}{*}{Open-source} &
%   YCB-Slide &
%   \multicolumn{1}{c}{DIGIT} &
%   180k &
%   Human &
%   SSL Representations \\
%  &
%   Touch and Go* &
%   \begin{tabular}[c]{@{}l@{}}Gelsight\\ (markers)\end{tabular} &
%   \textgreater{}13.9k &
%   Human &
%   SSL Representations \\
%  & ObjectFolder 2.0* & GelSight & \textgreater{}66k & Robot & SSL Representations \\
%  &
%   Feeling of Success &
%   \begin{tabular}[c]{@{}l@{}}Gelsight\\ (markers)\end{tabular} &
%   9.3k &
%   Robot &
%   Grasp Stability \\ \midrule
% \multirow{4}{*}{In-house data} &
%   YCB-Slide extension &
%   DIGIT &
%   180k &
%   Human &
%   SSL representations \\
%  & Shear load test  & DIGIT    &        490k            & Robot & Force \& Slip       \\
%  & Shear load test  & GelSight &        234k            & Robot & Force \& Slip       \\
%  & Object Sliding   & DIGIT    &         45k            & Robot & Pose Estimation     \\ \bottomrule
% \end{tabular}
% \caption{\textbf{Tactile Datasets} used for learning tactile representations and for their evaluation on downstream tasks. *For all datasets, we incorporate images corresponding to transitions from non-contact to contact.}
% \label{tab:datasets}
% \end{table}

==> tables/force_corr_digit.tex <==
\begin{table}[h]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Model          & Full dataset (50k) & $1/3$ dataset & $1/10$ dataset & \multicolumn{1}{l}{$1/100$ dataset} \\ \midrule
\ete   & 0.986        & 0.963         & 0.812          & 0.282                               \\
\mae   & 0.988        & 0.979         & 0.974          & 0.721                               \\
\textbf{\dino}  & \textbf{0.988}        & \textbf{0.985}         & \textbf{0.981}          & \textbf{0.833}                               \\
\ijepa & 0.986        & 0.964         & 0.880          & 0.614                               \\
\vjepa & 0.987        & 0.972         & 0.916          & 0.604                               \\ \bottomrule
\end{tabular}
\caption{DIGIT force correlation on flat probe}
\label{tab:force_corr_digit}
\end{table}

==> tables/force_corr_gelsight.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Model          & Full dataset & $1/3$ dataset & $1/10$ dataset & \multicolumn{1}{l}{$1/100$ dataset} \\ \midrule
\ete   & 0.961        & 0.921         & 0.821          & 0.505                               \\
\mae  & 0.974        & 0.968         & 0.950          & 0.650                               \\
\textbf{\dino}  & \textbf{0.980}        & \textbf{0.975}         & \textbf{0.956}          & \textbf{0.879}                               \\
\ijepa & 0.960        & 0.936         & 0.898          & 0.747                               \\
\vjepa) & 0.935        & 0.935         & 0.903          & 0.734                               \\ \bottomrule
\end{tabular}
\caption{GelSight correlation on flat probe data}
\label{tab:force_corr_gelsight}
\end{table}

==> tables/ssl_methods_comparison.tex <==
% SSL METHODS
\begin{table}[!t]
\GobbleLarge
\centering
\small
\begin{tabular}{@{}ccccc@{}}
\toprule
Model &
  Input &
  \begin{tabular}[c]{@{}c@{}}SSL\\ Framework\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Data\\ Augmentation\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Loss\\ Function\end{tabular} \\ \midrule
  \mae &
  \multirow{3}{*}{2 images $(h \times w \times 6)$} &
  Generative &
  Random Masking &
  \begin{tabular}[c]{@{}c@{}}$\Lv_2$ \\ pixel space\end{tabular} \\ [0.2cm]
  
  \dino &
   &
  Distillation &
  Block Masking &
  Cross-Entropy \\ [0.1cm]
  
  \ijepa &
   &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Joint-\\Embedding\\ Predictive\end{tabular}} &
  Multi-Block Masking &
  \begin{tabular}[c]{@{}c@{}}$\Lv_2$\\ latent space\end{tabular} \\ [0.1cm]
  \vjepa &
  4 images $(t \times h \times w \times 3)$ &
   &
  % \begin{tabular}[c]{@{}c@{}}Random Tube\\ Masking\end{tabular} &
  Random Tube Masking &
  \begin{tabular}[c]{@{}c@{}}$\Lv_1$\\ latent space\end{tabular} \\ \bottomrule
\end{tabular}
\caption{\textbf{Exploration of SSL Frameworks for Tactile Representation Learning.} We applied four SSL methods to determine the most suitable approach for learning representations in the domain of vision-based tactile images.}
\label{tab:ssl_methods_comparison}
\normalsize
\GobbleLarge
\end{table}
